Real-Time Visual Obstruction Detection in Surgical Augmented Reality

Surgical augmented reality (AR) can provide contextual guidance by overlaying virtual annotations, tool cues, and procedural information onto the surgical workspace. However, the virtual content may obstruct task-relevant real-world information, such as surgical instruments, and interfere with users' perception during time-sensitive surgical tasks. In this paper, we investigate visual obstruction detection for surgical AR and present a latency-aware pipeline that combines vision-language model (VLM)-based surgical-object recognition with segmentation-based obstruction reasoning. To reduce inference overhead, the system adopts a cascaded small-to-large VLM architecture with segmentation-guided early exiting and attention-based visual token pruning. The small VLM handles easy frames when its key-object prediction is supported by segmentation consistency, while difficult frames are forwarded to a large VLM with pruned visual tokens. We construct a pseudo-AR surgical obstruction detection benchmark by overlaying virtual content onto surgical-tool images and labeling whether the virtual content obstructs task-relevant instruments. Evaluation results show that the proposed system achieves 87.43% obstruction detection accuracy with an average end-to-end latency of 479 ms, reducing latency by 62.90% compared with a cloud large-model baseline. These results demonstrate the feasibility of latency-aware obstruction detection for surgical AR and motivate future work on dynamic surgical videos, multi-object scenes, and clinically grounded AR guidance content.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016
modified by Matt Brehmer, Feb 2024

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE VIS: Visualization & Visual Analytics (Short Papers, Posters)
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/5_discussion.tex <==
\section{Discussion and Future Work}

\label{sec:future}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{imgs/future.pdf}
    \vspace{-0.5cm}
    \caption{Future extension of the surgical AR obstruction detection pipeline. Recorded multi-object raw and AR videos are replayed by a video stream emulator to generate paired raw and AR frame streams. A frame-selection module filters out redundant frames to reduce unnecessary inference, while selected frames are forwarded to the obstruction detection module.}
    \vspace{-0.6cm}
    \label{fig:future_ext}
\end{figure}

\yx{

--------------------------------------------------------------------------

Yanming: Several thoughts.

I think we can structure this section around several limitations, using noindent\{textbf\{...\}\} to introduce each point. For each paragraph, we can first explain the current limitation and then discuss the corresponding future work. This may make the section more natural than directly listing future directions, since the future directions should grow out of the limitations rather than appear out of nowhere.

1. The scale of the dataset. Currently the dataset is pseudo AR and only has images. However, real AR surgical data are hard to obtain. This is why we want to use video generation for dataset collection.

2. The complexity of the task scenario. Currently our dataset only consider one surgical tool in each image. However, in real setup, the scenes can be quite complicated. This is why we will explore deeper into multi-object detection. To do this, we need to (1) "upgrade" the dataset to include multiple objects; (2) revise the current detection pipeline.

3. Further improve the efficiency of inference. Currently we call VLM for all the frames but this may not be fully necessary, especially when the user's view point is not changing violently. This is why we want o explore deeper into frame selection, where we...


--------------------------------------------------------------------------



}


\noindent{\textbf{Frame Selection}} Our current pipeline invokes the VLM on every candidate frame, which dominates end-to-end latency and energy cost on edge devices. A natural next step is to introduce a lightweight algorithmic filtering stage that screens frames before VLM inference, using inexpensive classical vision cues—such as feature matching and color-histogram comparison between consecutive frames—to discard clearly benign frames and reserve the VLM for suspicious ones. Such cues, however, operate at whole-frame granularity, and their coarse signals limit how precisely the filter can separate benign changes from adversarial ones. To sharpen this filtering stage, we plan to incorporate the pre-query evidence preservation mechanism, which distills incoming frames into fine-grained, tile-level visual evidence. Access to sub-frame information would allow the filter to reason about where in a frame changes occur rather than merely whether they occur, enabling more informed keep/drop decisions. Concretely, we envision (i) tile-level evidence scoring that localizes suspicious regions within otherwise-benign frames; (ii) a dynamically updated canvas that aggregates this fine-grained evidence across frames to provide richer context for filtering decisions; and (iii) coupling the preserved evidence with our token pruning strategy, so the VLM attends only to regions flagged by the evidence layer. We expect this design to substantially reduce VLM invocations while improving filtering precision, and plan to evaluate the trade-off between filter granularity and on-device overhead.



\noindent{\textbf{Video generation}}

\yx{In this part, we probably need to discuss several limitations of the current dataset: (1) static image; (2) small scale; (3) human annotation without validation.}

Building on our current study of surgical tool detection in AR-like scenarios, future work will explore AI-based video generation to support more realistic and clinically relevant surgical AR evaluation. Surgical AR is a promising direction for enhancing intraoperative visualization and providing surgeons with richer visual guidance. Beyond tool detection, future AR applications may involve anatomy labeling, lesion guidance, and procedure-specific visual cues that are closely aligned with real surgical needs.

To support this direction, AI-generated surgical videos could be used to synthesize specific surgical moments based on real surgical images. Compared with manually adding AR overlays to static images, video generation offers a more scalable way to create diverse AR scenarios with controllable virtual content. It also enables the construction of dynamic cases involving camera motion, changing viewpoints, tool movement, and temporary occlusions, which are important for evaluating AR perception systems in more realistic settings.

This approach is especially useful because real surgical videos are often difficult to collect at scale due to patient privacy considerations and limited operating room availability. By generating representative surgical scenes with clinically meaningful AR overlays, future datasets can better capture the visual complexity of real procedures while reducing dependence on large-scale real-world recordings. Representative examples are shown in~\cref{fig:generated}. Medical professional supervision will remain essential to ensure that the generated content is anatomically plausible, clinically relevant, and appropriate for surgical AR applications.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{imgs/generated.pdf}
    \vspace{-0.5cm}
    \caption{}
    \vspace{-0.6cm}
    \label{fig:generated}
\end{figure}

\noindent{\textbf{Multiple Object Detection}}
Extending the system to multiple object detection is an important direction for future work, since real operating rooms often contain several surgical tools and objects within the same scene. In such scenes, objects may appear close to each other, partially overlap, or become mutually occluded. These situations introduce additional complexity compared with the single-object setting studied in this work.

Addressing complex multiple-object detection scenarios requires more adaptive early exiting strategies. The current segmentation-guided early exiting method is designed to reduce redundant segmentation by identifying highly similar masks. The mechanism is effective for avoiding repeated detections in single-object cases. However, when moving toward multiple-object scenarios, overlapping tools or closely positioned objects may naturally produce masks with higher overlap. Therefore, future methods should distinguish between redundant masks and valid overlapping objects more carefully.

To support this goal, future work will refine early exiting strategies that incorporate additional information beyond mask-level IoU, such as spatial relationships and prompt consistency. These cues could help improve robustness in complex scenes with multiple objects.

This direction would improve the system’s applicability to realistic surgical AR scenarios. In these scenarios, multiple tools, anatomical structures, hands, and virtual overlays may appear at the same time. By extending the framework to multiple-object detection, future AR-assisted perception systems can better reflect the visual complexity of real operating room environments.

